Unbiased determination of polarized parton distributions and their uncertainties

We present a determination of a set of polarized parton distributions (PDFs) of the nucleon, at next-to-leading order, from a global set of longitudinally polarized deep-inelastic scattering data: NNPDFpol1.0. The determination is based on the NNPDF methodology: a Monte Carlo approach, with neural networks used as unbiased interpolants, previously applied to the determination of unpolarized parton distributions, and designed to provide a faithful and statistically sound representation of PDF uncertainties. We present our dataset, its statistical features, and its Monte Carlo representation. We summarize the technique used to solve the polarized evolution equations and its benchmarking, and the method used to compute physical observables. We review the NNPDF methodology for parametrization and fitting of neural networks, the algorithm used to determine the optimal fit, and its adaptation to the polarized case. We finally present our set of polarized parton distributions. We discuss its statistical properties, test for its stability upon various modifications of the fitting procedure, and compare it to other recent polarized parton sets, and in particular obtain predictions for polarized first moments of PDFs based on it. We find that the uncertainties on the gluon, and to a lesser extent the strange PDF, were substantially underestimated in previous determinations.

==> exps-err.tex <==
 \begin{tabular}{|ll|c|c|c|}
 \hline
 Experiment & Set
 & $\langle\delta{A_1}_{\mbox{\tiny s}}\rangle$
 & $\langle\delta{A_1}_{\mbox{\tiny c}}\rangle$
 & $\langle\delta{A_1}_{\mbox{\tiny tot}}\rangle$\\
 \hline
 \hline
 \multicolumn{2}{|l|}{EMC       } & & & \\
 & EMC-A1P    &        0.081 &        0.024 &        0.085\\
 \hline
 \multicolumn{2}{|l|}{SMC       } & & & \\
 & SMC-A1P    &        0.032 (0.032) &        -- (--) &        0.032 (0.032)\\
 & SMC-A1D    &        0.036 (0.036) &        -- (--) &        0.036 (0.036)\\
 \hline
 \multicolumn{2}{|l|}{SMClowx   } & & & \\
 & SMClx-A1P  &        0.034 (0.045) &        -- (--) &        0.034 (0.045)\\
 & SMClx-A1D  &        0.070 (0.093) &        -- (--) &        0.070 (0.093)\\
 \hline
 \multicolumn{2}{|l|}{E143      } & & & \\
 & E143-A1P   &        0.064 (0.039) &        0.012 (0.011) &        0.065 (0.041)\\
 & E143-A1D   &        0.094 (0.054) &        0.008 (0.007) &        0.094 (0.054)\\
 \hline
 \multicolumn{2}{|l|}{E154      } & & & \\
 & E154-A1N   &        0.063 &        --  &        0.063\\
 \hline
 \multicolumn{2}{|l|}{E155      } & & & \\
 & E155-G1P   &        0.039 (0.034) &        -- (--) &        0.039 (0.034)\\
 & E155-G1N   &        0.174 (0.130) &        -- (--) &        0.174 (0.130)\\
 \hline
 \multicolumn{2}{|l|}{COMPASS-D } & & & \\
 & CMP07-A1D  &        0.025 &        --  &        0.025\\
 \hline
 \multicolumn{2}{|l|}{COMPASS-P } & & & \\
 & CMP10-A1P  &        0.030 &        --  &        0.030\\
 \hline
 \multicolumn{2}{|l|}{HERMES97  } & & & \\
 & HER97-A1N  &        0.123 (0.090) &        -- (--) &        0.123 (0.090)\\
 \hline
 \multicolumn{2}{|l|}{HERMES    } & & & \\
 & HER-A1P    &        0.146 (0.062) &        -- (--) &        0.146 (0.062)\\
 & HER-A1D    &        0.103 (0.037) &        -- (--) &        0.103 (0.037)\\
 \hline
 \end{tabular}


==> sec-app.tex <==
\section{Kernels for Physical Observables}
\label{sec:kernels}
\def\nn{\nonumber}
\def\GS{\Gamma_{\rm S}}
\def\GNS{\Gamma_{\rm NS}}
\def\half{\smallfrac{1}{2}}
\def\ESp{E_{\rm S}^+} 
\def\ESm{E_{\rm S}^-} 
\def\ENSp{E_{\rm NS}^+} 
\def\ENSm{E_{\rm NS}^-} 

In this appendix we give the expression of
the polarized structure functions $g_1(x,Q^2)$ in terms
of the combinations of PDFs used in
Sec.~\ref{sec:fact}. We follow the notation of
Ref.~\cite{Ball:2008by}.  The expressions below can be used with
evolution kernels and coefficients evaluated at any order in
perturbation theory. At present, polarized evolution kernels
$\GNS^{\pm,v}$ and $\GS^{ij}$, $i,j = q,g$, as described in 
Ref.~\cite{Ball:2008by}, are available
at NLO~\cite{Mertig:1995ny},\cite{Vogelsang:1996im}.
Partial NNLO results are given in Ref.~\cite{Vogt:2008yw}. The DIS coefficient
functions are known up to NNLO~\cite{Zijlstra:1993sh}.

Throughout this section we use a condensed notation in which the 
arguments of $f_i$, $F_I$, $\Gamma$, $C$ and $K$ are 
all suppressed: parton distributions evaluated at $Q_0^2$ are denoted by
a subscript $0$, e.g. $\Delta \Sigma_0\equiv\Delta 
\Sigma(x,Q_0^2)$. We will assume 
throughout that $Q_0^2=1$ GeV$^2$. Heavy quark
parton distributions are radiatively generated 
as described in Sect.~\ref{sec:fact}. 
Target mass corrections are included in the kernels using 
the procedure described in Sect.~\ref{sec:tmc}.

The datasets we include in our analysis include measurements 
of $g_1^p$, $g_1^d$ and $g_1^n$. These observables 
can be written in terms of the
linear combinations of polarized parton densities:
in the quark model, the proton polarized structure function 
has been shown in Eq.~(\ref{g1p-parton}), while
in the PDF evolution basis it reads
\be
\label{eq:g1p}
  g_1^p = \smallfrac{1}{2}
\sum_{i=1}^{n_f} e_i^2 \Delta q_i^+ = \smallfrac{1}{2}\lbrace\smallfrac{5}{18}
\Delta \Sigma 
             + \smallfrac{1}{6} \Delta T_3
                + \smallfrac{1}{18} (\Delta T_8 - \Delta T_{15})
        + \smallfrac{1}{30} (\Delta  T_{24}- \Delta T_{35})\rbrace\ ,
\ee
where $e_i$ are the quark charges 
($\smallfrac{2}{3}$ for $u,c,t$, $-\smallfrac{1}{3}$ for $d,s,b$).  
The deuteron polarized structure function can be written as
\be
  \label{eq:g1d}
 g_1^d = \smallfrac{1}{2}\lbrace\smallfrac{5}{18}
\Delta \Sigma 
%             + \smallfrac{1}{6} \Delta T_3
                + \smallfrac{1}{18} (\Delta T_8 - \Delta T_{15})
        + \smallfrac{1}{30} (\Delta  T_{24}- \Delta T_{35})\rbrace\ ,
\ee
while the neutron polarized structure function is given
in terms of the proton and deuteron ones as
\be
  \label{eq:g1n}
  g_1^n = 2\frac{g_1^d}{1-1.5\omega_D}-g_1^p\ ,
\ee
with $\omega_D=0.05$ the probability that the deuteron is found
in a D state.

In perturbative QCD, we have
\begin{eqnarray}
  \label{eq:f2pdfcomp}
  g_1^p &=& \lbrace \smallfrac{5}{18}\Delta  C^s_{2,q}\otimes \Delta \Sigma 
             + \smallfrac{1}{6}\Delta  C_{2,q}\otimes( \Delta  T_3
                + \smallfrac{1}{3} (\Delta  T_8 - \Delta  T_{15})
        + \smallfrac{1}{5} (\Delta  T_{24}-\Delta T_{35}))\nn\\
 &&\qquad\qquad\qquad\qquad\qquad\qquad 
+ {\langle e_q^2\rangle} \Delta  C_{2,g}\otimes \Delta g\rbrace ,\\
  \label{eq:f2pdfcomd}
  g_1^d &=& \lbrace \smallfrac{5}{18}\Delta  C^s_{2,q}\otimes \Delta \Sigma 
             + \smallfrac{1}{6}\Delta  C_{2,q}\otimes(
          \smallfrac{1}{3} (\Delta  T_8 - \Delta  T_{15})
        + \smallfrac{1}{5} (\Delta  T_{24}-\Delta T_{35})) \nn\\
 &&\qquad\qquad\qquad\qquad\qquad\qquad      + {\langle e_q^2\rangle}  \Delta  C_{2,g}\otimes \Delta g\rbrace \ ,
\end{eqnarray}
where $\otimes$ denotes the Mellin convolution, 
and ${\langle e_q^2\rangle}$ is defined as
\be
\label{ceenf}
 {\langle e_q^2\rangle} = \smallfrac{1}{n_f}\sum_{i=1}^{n_f} e_i^2,
\ee
whith $n_f$ the number of active flavours: 
${\langle e_q^2\rangle} = \smallfrac{2}{9},
\smallfrac{5}{18},\smallfrac{11}{45},\smallfrac{5}{18}$ for $n_f = 3,4,5,6$.
We can thus write
 \bea
\label{Kg1pp}
  g_1^p&=& \lbrace 
        K_{{\rm g1},\Delta\Sigma}\otimes \Delta\Sigma_0 
+K_{{\rm g1},\Delta g} \otimes \Delta g_0 
+K_{{\rm g1},+} \otimes  \left(\Delta T_{3,0}
                + \smallfrac{1}{3}\Delta T_{8,0}\right)\rbrace\ ,\\
\label{Kg1dd}
  g_1^d&=& \lbrace 
        K_{{\rm g1},\Delta\Sigma}\otimes \Delta\Sigma_0 
+K_{{\rm g1},\Delta g} \otimes \Delta g_0 
+K_{{\rm g1},+} \otimes  
   \smallfrac{1}{3}\Delta T_{8,0}
\rbrace\ ,
 \eea
where the explicit expressions (in Mellin space) for the polarized evolution kernels are
\begin{eqnarray}
\label{eq:Kf2S} 
K_{{\rm g1},\Delta\Sigma}&=&\smallfrac{5}{18} \Delta C^s_{2,q}\GS^{qq}
-\smallfrac{1}{18} \Delta C_{2,q}\GS^{15,q}
+\smallfrac{1}{30} \Delta C_{2,q}(\GS^{24,q}-\GS^{35,q})
+{\langle e_q^2\rangle} \Delta C_{2,g}\GS^{gq}\ ,\\
  \label{eq:Kf2g}
K_{{\rm g1},\Delta g}&=&\smallfrac{5}{18} \Delta C^s_{2,q}\GS^{qg}
-\smallfrac{1}{18} \Delta C_{2,q}\GS^{15,g}
+\smallfrac{1}{30} \Delta C_{2,q}(\GS^{24,g}-\GS^{35,g})
+{\langle e_q^2\rangle} \Delta C_{2,g}\GS^{gg}\ ,\\
  \label{eq:Kf2T}
 K_{{\rm g1},+}&=& \smallfrac{1}{6} \Delta C_{2,q}\GNS^+\ .
    \end{eqnarray}


%----------------------------------------------------


==> sec-pdferr.tex <==
%----------------------------------------------------------------

\section{Computation  of PDF uncertainties}
\label{sec:app-pdferr}

In this appendix we briefly review the main formulae
to compute PDF uncertainties.
Available methods for the determination of PDF uncertainties 
fall broadly into two distinct categories, which we shall refer to as
the Hessian method 
and the {Monte Carlo method}.\footnote{
The Monte Carlo method to PDF error determination is the default
in NNPDF, but it has also been used by the MSTW~\cite{Watt:2012tq}
and HERAPDF~\cite{Jung:2009eq}
collaborations in the unpolarized case.}
In both cases, sets of polarized PDFs with uncertainties are given as
an ensemble of $N_{\rm set}$ sets of PDFs, 
\be\{ \Delta q^{(k)} \} \ , \qquad k=0,\ldots,N_{\rm set}.
\ee 
Conventionally the PDF set $\Delta q^{(0)}$ corresponds to a ``central'' set. 

Within the Monte Carlo approach, 
the expectation value of any function 
$ \mathcal{F} [ \{  \Delta q \}]$ which depends
on the PDFs is computed as an average over the ensemble of PDFs, using
the master formula
\be
\label{masterave}
\la \mathcal{F} [ \{  \Delta q \}] \ra
= \frac{1}{N_{\rm set}} \sum_{k=1}^{N_{\rm set}}
\mathcal{F} [ \{  \Delta q^{(k)} \}],
\ee
where $N_{\rm set}=N_{\rm rep}$ is the number of sets of PDFs in the ensemble,
equal to the number of replicas. 
The associated uncertainty is found as the standard deviation of the
sample, according to the usual formula
\bea
\sigma_{\mathcal{F}} 
&=& \left[ \frac{N_{\rm set}}{N_{\rm set}-1}   
\lp \la \mathcal{F} [ \{  \Delta q \}]^2\ra 
-   \la \mathcal{F} [ \{  \Delta q \}] \ra^2 
\rp \right]^{1/2}\nn\\
&=& \left[ \frac{1}{N_{\rm set}-1}
\sum_{k=1}^{N_{\rm set}}   
\lp \mathcal{F} [ \{  \Delta q^{(k)} \}] 
-   \la \mathcal{F} [ \{  \Delta q \}] \ra\rp^2 
 \right]^{1/2}.
\label{mastersig}
\eea
These formulae may also be used for the determination of central values and
uncertainties of the parton distribution themselves, in which case the
functional $\mathcal{F}$ is identified with the parton distribution $\Delta q$:  
$\mathcal{F}[ \{ \Delta q\}]\equiv \Delta q$.

Alternatively, for a Monte Carlo PDF set, one can compute PDF
uncertainties as confidence level (CL) intervals. For a $(1-2p)\%$
Confidence Level interval, one just needs to order the
$N_{\rm set}$ obtained from each of the replicas of the sample,
and discard the $p$ lower and higher replicas. For example, if 
$N_{\rm set}=100$, the 68 \% Confidence Level is obtained by 
removing from the sample the 16 higher and 16 lower replicas
for a given cross section (or PDF set in a given point in
$(x,Q^2)$): the remaining replicas define the 68 \% Confidence Level
interval. When the Gaussian linear approximation holds the
68~\% CL will be very similar to the 1--$\sigma$ PDF error
Eq.~(\ref{mastersig}), but in other regions where the Gaussian
behavour breaks down differences can be sizable,
as shown in Fig.~\ref{fig:pdfcl68}.

In the Hessian method, used in all recent
polarized PDF sets~\cite{deFlorian:2009vb,Leader:2010rb,Hirai:2008aj,Blumlein:2010rn}, the central set is a best fit set
of PDFs, which thus provides the central value for PDFs
themselves.
 The central value of any quantity $\mathcal{F}[ \{  \Delta q
\}]$ is obtained in this method
by evaluating it as a function of the central set: 
\be
\label{naiveav}
\mathcal{F}^{(0)}=
\mathcal{F}[ \{   \Delta q^{(0)} \}].
\ee
The determination of uncertainties with  the Hessian method is
based on the idea that sets $  \Delta q^{(k)}$ with $k>0$ provide upper and
lower variations (for even and odd values of $k$)
away from the central set  $  \Delta q^{(0)}$ which correspond to eigenvectors
in parameter space. 
The 1--$\sigma$ uncertainty is then found by adding in quadrature 
these variations:
\be
\label{hepdataerr}
\sigma_{\mathcal{F} }^{\rm hessian} = \frac{1}{2}\lp 
\sum_{k=1}^{N_{\rm set}/2} 
\lp \mathcal{F} [ \{  \Delta q^{(2k-1)} \}]
- \mathcal{F} [ \{  \Delta q^{(2k)} \}] \rp^2\rp^{1/2}.
\ee
The resulting error could be interpreted as 1--$\sigma$ error, however in many
cases the tolerances used in the PDF error definition are larger
than the textbook value, $\Delta\chi^2 \gg 1$, and thus the statistical
interpretation of the results is hindered.



To conclude, let us discuss how to obtain the
``central value'' for a Monte Carlo PDF set.
In the Monte Carlo method, 
the central values of any quantity  $\mathcal{F}[ \{ \Delta q
\}]$ are instead given by  Eq.~(\ref{masterave}). Therefore, 
the central
value for PDFs themselves is given by 
 \be
\label{mcav}
\Delta q^{(0)} \equiv \la  \Delta q \ra = \frac{1}{N_{\rm set}}
\sum_{k=1}^{N_{\rm set}} \Delta q^{(k)} \ .
\ee
This set is provided as set $\Delta q^{(0)}$ in the
{\tt NNPDFpol1.0} PDFs. Hence, in the Monte Carlo method the central (best
fit) PDF is obtained as an average of the replica  best fits.
However, for any quantity 
$\mathcal{F}[ \{  \Delta q \}]$ which 
depends nonlinearly on the PDFs, such as cross section asymmetries in
polarized hadronic collisions,
\be
\label{linearav}
\la \mathcal{F} [ \{  \Delta q \}] \ra 
\not= 
 \mathcal{F} [\{  \Delta q^{(0)}\}] .
\ee
Hence,
Eq.~(\ref{masterave}) must be used  for the determination of the
central value, and using  the  set  $q^{(0)}$ is not 
recommended. However, for a quantity that does depend linearly on the
PDFs, such as a DIS polarized structure function, Eq.~(\ref{naiveav}) with the
central PDFs Eq.~(\ref{mcav}) gives the
same result as Eq.~(\ref{masterave}), and thus it may be used
also with the Monte Carlo method (but this is not true for
example for cross section in polarized hadronic collisions).
Note that set $\Delta q^{(0)}$ should not be included when
computing an average with Eq.~(\ref{masterave}), because it is 
itself already an average.



